Layer-adaptive sparsity for the Magnitude-based Pruning

Recent discoveries on neural network pruning reveal that, with a carefully chosen layerwise sparsity, a simple magnitude-based pruning achieves state-of-the-art tradeoff between sparsity and performance. However, without a clear consensus on "how to choose," the layerwise sparsities are mostly selected algorithm-by-algorithm, often resorting to handcrafted heuristics or an extensive hyperparameter search. To fill this gap, we propose a novel importance score for global pruning, coined layer-adaptive magnitude-based pruning (LAMP) score; the score is a rescaled version of weight magnitude that incorporates the model-level $\ell_2$ distortion incurred by pruning, and does not require any hyperparameter tuning or heavy computation. Under various image classification setups, LAMP consistently outperforms popular existing schemes for layerwise sparsity selection. Furthermore, we observe that LAMP continues to outperform baselines even in weight-rewinding setups, while the connectivity-oriented layerwise sparsity (the strongest baseline overall) performs worse than a simple global magnitude-based pruning in this case. Code: https://github.com/jaeho-lee/layer-adaptive-sparsity

==> figures/app_prunefrac.tex <==
\begin{figure*}[ht!]
\centering
 \subfigure[Global MP w/ normal]{
 \centering
 \includegraphics[width=0.24\textwidth]{figs/global_normal2.pdf}
 }
 %
 \hspace{-0.2in}
 \subfigure[Global MP w/ uniform]{
 \centering
 \includegraphics[width=0.24\textwidth]{figs/global_uniform2.pdf}
 }
 %
 \subfigure[MPDR w/ normal]{
 \centering
 \includegraphics[width=0.24\textwidth]{figs/mpdr_normal2.pdf}
 }
 %
 \subfigure[MPDR w/ uniform]{
 \centering
 \includegraphics[width=0.24\textwidth]{figs/mpdr_uniform2.pdf}
 }
\caption{Sparsity trends of transformers whose first and last layers are initialized with either $\mathsf{Unif}(-0.1,0.1)$ or $\cN(0,1)$, pruned by either global MP or MPDR.}
 \label{fig:globalfail}
\end{figure*}


==> tables_new/resnet18.tex <==
\begin{table*}[!ht]
\caption{Test accuracies of ResNet-18 iteratively pruned and trained on CIFAR-10. Bold denotes the pruning scheme with accuracy within one standard deviation from the highest.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrr}
\toprule
Surv. weights & 6.87\% & 4.40\% & 2.81\% & 1.80\% & 1.15\% & 0.74\% & 0.47\% & 0.30\% & 0.19\% & 0.12\%\\
\midrule
Global& 92.74\stdv{0.22}& 92.49\stdv{0.18}& 92.18\stdv{0.11}& 91.27\stdv{0.10}& 89.78\stdv{0.36}& 86.80\stdv{1.55}& 83.57\stdv{2.44}& 61.25\stdv{28.40}& 60.72\stdv{23.04}& 29.84\stdv{26.45}\\
Uniform & 92.94\stdv{0.21}& 92.59\stdv{0.21}& 91.99\stdv{0.23}& 90.89\stdv{0.27}& 89.67\stdv{0.11}& 87.71\stdv{0.27}& 84.90\stdv{0.73}& 61.85\stdv{29.20}& 20.53\stdv{11.13}& 11.42\stdv{2.21}\\
Uniform+& 92.88\stdv{0.18}& 92.53\stdv{0.17}& 92.07\stdv{0.18}& 91.29\stdv{0.20}& 90.08\stdv{0.18}& 88.67\stdv{0.40}& 86.67\stdv{0.16}& 83.98\stdv{0.37}& 77.13\stdv{3.32}& 44.69\stdv{30.24}\\
Erd\H{o}s-Rényi ker.& {\bf93.29}\stdv{0.27}& {\bf93.05}\stdv{0.11}& {\bf92.90}\stdv{0.18}& {\bf92.45}\stdv{0.14}& 91.86\stdv{0.25}& 90.69\stdv{0.22}& 89.52\stdv{0.22}& 88.16\stdv{0.28}& 85.71\stdv{0.38}& 81.87\stdv{0.35}\\
\midrule
\rowcolor{GGray}LAMP (Ours)& {\bf93.24}\stdv{0.25}& {\bf93.18}\stdv{0.15}& {\bf92.96}\stdv{0.22}& {\bf92.68}\stdv{0.31}& {\bf92.12}\stdv{0.19}& {\bf91.40}\stdv{0.35}& {\bf90.54}\stdv{0.14}& {\bf88.99}\stdv{0.22}& {\bf87.24}\stdv{0.23}& {\bf84.61}\stdv{0.48}\\
\bottomrule
\end{tabular}}
\end{table*}

==> tables_new/restrictedimagenet.tex <==
\begin{table*}[!ht]
\caption{Test accuracies of ResNet-34 iteratively pruned and trained on RestrictedImageNet. Bold denotes the pruning scheme with accuracy within one standard deviation from the highest.} \label{table:restrictedimagenet}
%\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
\toprule
Surv. weights & 6.87\% & 3.52\% & 1.80\% & 0.92\% & 0.47\% & 0.24\% & 0.12\%\\
\midrule
Global& \textbf{94.62}& 93.81& 93.24& 91.90& 89.62& 88.19& 84.62\\
Uniform & 94.00& 93.86& 92.05& 91.00& 86.62& 73.43& 36.38\\
Uniform+ & 94.00& 93.86& 92.05& 91.00& 86.62& 73.43& 36.38\\
Erd\H{o}s-Rényi ker.& 94.48& 93.86& \textbf{94.05}& 93.33& 92.19& 90.76& 88.28\\
\midrule
\rowcolor{GGray}LAMP (Ours)& 94.38& \textbf{94.43}& 93.90& \textbf{93.57}& \textbf{92.90}& \textbf{91.76}& \textbf{89.86}\\
\bottomrule
\end{tabular}%}
\end{table*}

==> txts/3_lamp.tex <==
\section{Layer-adaptive magnitude-based pruning (LAMP)} \label{sec:lamp}
We now formally introduce the Layer-Adaptive Magnitude-Based Pruning (LAMP) score. Consider a depth-$d$ feedforward neural network with weight tensors $W_1,\ldots,W_d$ associated to each fully-connected/convolutional layer. For each layer, we assume (without loss of generality) that the weights are sorted in an ascending order according to the given index map, i.e., $|W_i[u]| \le |W_i[v]|$ holds whenever $u < v$. The LAMP score is then defined as
\begin{align}
    \mathsf{score}_i(u) \deq \frac{W_i^2[u]}{\sum_{v \geq u} W_i^2[v]}. \label{eq:lamp_score}
\end{align}
Informally, the LAMP score (Eq.~\ref{eq:lamp_score}) measures the relative importance of a connection among all \textit{surviving connections} belonging to the same layer. We note that, as a consequence, two connections with identical weight magnitudes have different LAMP scores, depending on the index map.

Once the LAMP score is computed, we globally prune the connections with smallest LAMP scores until the desired global sparsity constraint is met; the procedure is equivalent to performing MP with an automatically selected layerwise sparsity. To see this, it suffices to check that
\begin{align}
    W_i^2[u] > W_i^2[v] \Rightarrow \score_{i}(u) > \score_i(v) \label{eq:equiv_mp}
\end{align}
holds for any layer $i \in \{1,\ldots,d\}$. From the definition of the LAMP score (Eq.~\ref{eq:lamp_score}), it is easy to see that the logical relation \eqref{eq:equiv_mp} holds. Indeed, for the weight with larger magnitude, the denominator of Eq.~\ref{eq:lamp_score} is smaller, while the numerator is larger.

We also note that the LAMP score is \text{easy-to-use}. Similar to the vanilla MP, the LAMP score does not have any hyperparameter to be tuned, and is easily implementable via elementary tensor operations. Furthermore, computing the LAMP score imposes only a minimal computational overhead; the sorting of squared weight magnitudes required to compute the denominator in Eq.~\ref{eq:lamp_score} is already a part of typical vanilla MP algorithms. For more discussions, see \cref{app:computation}.

\subsection{Design principle: Minimizing output $\ell_2$ distortion} \label{ssec:lamp_motive}
To motivate LAMP, we begin by viewing the layerwise MP as a minimization of pruning-incurred $\ell_2$ distortion in layer output, given the worst-case (unit) input signal. Then, we proceed to consider the model-level distortion, motivating the LAMP score (Eq.~\ref{eq:lamp_score}). For a formal discussion, consider a depth-$d$ feedforward neural network, whose output given an input $x$ is
\begin{align}
f(x;W_{1:d}) = W_d \sigma \big( W_{d-1} \sigma \big( \cdots W_{2} \sigma \big( W_1 x\big) \cdots \big)\label{eq:feedforward},
\end{align}
where $\sigma$ denotes the ReLU activation and $W_i$ denotes the linear transformation corresponding to $i$-th layer. For a fully-connected layer, $W_i$ is its weight matrix. For a two-dimensional convolutional layer, $W_i$ is a doubly block circulant matrix built with the kernel tensor \citep{sedghi19}. We focus on fully-connected layers for a simple presentation, but the extension to convolutional layers is straightforward, as the magnitude ranking for a doubly block circulant matrix is identical to the magnitude ranking of the convolutional kernel.

\textbf{MP: layerwise distortion minimization.}
We first focus on a single fully-connected layer. Let $\xi_i$ be the input to the $i$-th layer and $\widetilde{W}_i$ be a pruned version of $W_i$. We aim to minimize the output distortion from pruning, as measured by the $\ell_2$ distance $\|W_i\xi_i - \widetilde{W}_i\xi_i\|_2$. Minimizing $\ell_2$ distortion for the worst-case input signal is equivalent to minimizing the spectral norm distortion
\begin{align}
    \min_{\widetilde{W}_i} \sup_{\|\xi_i\|_2 \leq 1} \|W_i \xi_i - \widetilde{W}_i \xi_i\|_2 = \min_{\widetilde{W}_i} \|W_i - \widetilde{W}_i\|, \label{eq:mp_minimax}
\end{align}
where the search space for $\widetilde{W}_i$ is determined by some given sparsity constraint. The optimization \eqref{eq:mp_minimax} can be relaxed (via Cauchy-Schwarz inequality) to a Frobenius distortion minimization
\begin{align}
    \min_{M_i: \|M_i\|_0 \leq \kappa_i} \|W_i - M_i \odot W_i\| \le \min_{M_i: \|M_i\|_0 \leq \kappa} \|W_i - M_i \odot W_i\|_F, \label{eq:mp_opt}
\end{align}
where $M_i$ is a binary matrix, i.e. having only $0$s and $1$s as its entries, $\|\cdot\|_0$ denotes the entrywise $\ell_0$ norm, and $\kappa$ denotes the given sparsity constraint. We now observe that the (layerwise) MP gives an optimal solution for the optimization \eqref{eq:mp_opt}. Indeed, the squared Frobenius distortion is simply a sum of pruned squared weight magnitudes, and the optimal decision is to keep $\kappa_i$ weights with the largest weight magnitudes.

\textbf{LAMP: greedy minimization of model distortion.} Now we step further to consider the $\ell_2$ distortion from pruning depth-$d$ neural network. Namely, we want to minimize
\begin{align}
    \min_{\widetilde{W}_{1:d}}\sup_{\|x\|_2\leq 1} \|f(x;W_{1:d}) - f(x;\widetilde{W}_{1:d}),\|_2, \label{eq:model_distortion}
\end{align}
where the search space of $\widetilde{W}_{1:d}$ is characterized by the given global sparsity constraint. Due to the non-linearities introduced by activation functions, unfortunately, it is difficult to solve Eq.~\ref{eq:model_distortion} exactly. Instead, we consider the following greedy procedure: At each step, (1) we compute a \textit{damage score} (not identical to the LAMP score, will be explained shortly) that approximates the distortion incurred by pruning the target weight. (2) Then, we remove a \textit{single connection} with the smallest score. (3) Finally, we go back to step (1) and re-compute the scores based on the \textit{pruned model}.

To approximate the distortion incurred by pruning a weight in $i$-th layer, we use a popular relaxation from the generalization theory literature (see, e.g., \citet{neyshabur15}). Namely, we use the fact that the ReLU activation is $1$-Lipschitz and has zero-in-zero-out property\footnote{i.e. $\sigma(0) = 0$.} to arrive at
\begin{align}
    &\sup_{\|x\|_2\leq 1} \|f(x;W_{1:d}) - f(x;W_{1:i-1}, \widetilde{W}_i,W_{i+1:d})\|_2 \leq \frac{\|W_i - \widetilde{W}_i\|_F}{\|W_i\|_F} \cdot \left(\prod_{j = 1}^d \|W_j\|_F\right). \label{eq:peeling_bound}
\end{align}
A (straightforward) proof of Ineq.~\ref{eq:peeling_bound} is given in \cref{app:inequality}. Inspired by this relaxation, we use the right-hand side as the \textit{damage score}, which should be re-computed every time after pruning each connection. Luckily, the product term $\prod_{j=1}^d \|W_j\|_F$ does not affect the pruning decision at each pruning step, and what we need to re-compute at each time step is the denominator $\|W_i\|_F$. Even more luckily, this quantity can be pre-computed at a single step by replacing $\|W_i\|_F$ with a cumulative sum $\sum_{v\ge u} W_i^2[v]$ for each element $u$ in $W_i$. By the replacement, we arrive at the LAMP score (Eq.~\ref{eq:lamp_score}), which does not require a re-computation after pruning every single connection.


